Universal Convexification via Risk-Aversion

We develop a framework for convexifying a fairly general class of optimization problems. Under additional assumptions, we analyze the suboptimality of the solution to the convexified problem relative to the original nonconvex problem and prove additive approximation guarantees. We then develop algorithms based on stochastic gradient methods to solve the resulting optimization problems and show bounds on convergence rates. %We show a simple application of this framework to supervised learning, where one can perform integration explicitly and can use standard (non-stochastic) optimization algorithms with better convergence guarantees. We then extend this framework to apply to a general class of discrete-time dynamical systems. In this context, our convexification approach falls under the well-studied paradigm of risk-sensitive Markov Decision Processes. We derive the first known model-based and model-free policy gradient optimization algorithms with guaranteed convergence to the optimal solution. Finally, we present numerical results validating our formulation in different applications.

==> Applications.tex <==


\section{Applications}

\subsection{Structured Controller Design for Linear Systems}

Consider a linear dynamical systems $\s_{t+1}=A_t\s_t+B_t\yg_t,\s_1=0$ (we assume a noiseless system here for brevity). We seek to synthesize linear state feedback policies $\ug_t=K_t\s_t$ with structural constraints $\Kb \in \C$. If the state costs are quadratic: $\cost(\s_t)=\frac{\tran{\s_t}\costx_t\s_t}{2}$, the expectations in \eqref{eq:OptC} can be computed analytically. We can write down

\[\traj=\begin{pmatrix} \s_1 \\ \s_2 \\ \vdots \\ \s_{\Nh} \end{pmatrix} = \underbrace{\begin{pmatrix} 0 & 0 & 0 & \ldots & 0\\B_1 & 0 & 0 & \ldots & 0 \\
A_1B_1 & B_2 & 0 & \ldots & 0 \\ \vdots & \vdots & \vdots & \vdots & \vdots \\ \prod_{t=\Nh-1}^{1} A_t B_1 & \prod_{t=\Nh-1}^{2} A_t B_2 & \prod_{t=\Nh-1}^{3} A_t B_3 & \ldots & B_{\Nh-1}\end{pmatrix}}_{\M}\begin{pmatrix} \yg_1  \\ \vdots \\ \yg_{\Nh-1} \end{pmatrix} =\M\ytraj\]
where $\M$ is an $\R^{\Nh\ns \times (\Nh-1)\nc}$ matrix that is independent of $\Kb$. Also, define:

\begin{align*}
\mathcal{S}=\begin{pmatrix} S_1 & 0 & \ldots & 0 \\ 0 & S_2 & \ldots & 0 \\ \vdots & \vdots & \vdots & \vdots \\ 0 & 0 & \ldots & S_{\Nh-1} \end{pmatrix} \in \R^{m(\Nh-1) \times m(\Nh-1)},\mathcal{K} = \begin{pmatrix} K_1 & 0 & \ldots & 0 & 0\\ 0 & K_2 & \ldots & 0 & 0\\ \vdots & \vdots & \vdots & \vdots & \vdots \\ 0 & 0 & \ldots & K_{\Nh-1} & 0\end{pmatrix} \in \R^{m(\Nh-1) \times n\Nh} \\
\mathcal{R}=\begin{pmatrix} R_1 & 0 & \ldots & 0 \\ 0 & R_2 & \ldots & 0 \\ \vdots & \vdots & \vdots & \vdots \\ 0 & 0 & \ldots & R_{\Nh-1} \end{pmatrix} \in \R^{m(\Nh-1) \times m(\Nh-1)},\mathcal{Q} = \begin{pmatrix} Q_1 & 0 & \ldots & 0\\ 0 & Q_2 & \ldots & 0\\ \vdots & \vdots & \vdots & \vdots \\ 0 & 0 & \ldots & Q_{\Nh}\end{pmatrix} \in \R^{n\Nh \times n\Nh}
\end{align*}

Let $c=\sqrt{\powb{2\pi}{\nc (\Nh-1)}\prod_{t=1}^{\Nh-1} \detb{\Unoise_t}}$. The expectation becomes
\begin{align*}
& \frac{1}{c}\int \expb{-\sum_{t=1}^{\Nh-1} \frac{\norm{\yg_t-K_t\s_t}_{\Unoisei_t}^2}{2}}\expb{\risk\br{\sum_{t=1}^{\Nh-1} \frac{\tran{\s_t}\br{Q_t+\tran{K_t}R_tK_t}\s_t}{2}+\frac{\tran{\s_{\Nh}}Q_{\Nh}\s_{\Nh}}{2}}}\diff{\ytraj} \\
& = \frac{1}{c}\int \expb{-\sum_{t=1}^{\Nh-1} \frac{\norm{\yg_t-K_t\s_t}_{\Unoisei_t}^2}{2}}{\expb{\risk\br{\sum_{t=1}^{\Nh-1} \frac{\tran{\s_t}\br{Q_t+\tran{K_t}R_tK_t}\s_t}{2}+\frac{\tran{\s_{\Nh}}Q_{\Nh}\s_{\Nh}}{2}}}}\diff{\ytraj} \\
& = \frac{1}{c}\int \expb{-\frac{1}{2}\tran{\ytraj}\mathcal{S}\ytraj+\tran{\ytraj}\mathcal{S}\mathcal{K}\traj-\frac{1}{2}\tran{\traj}\tran{\mathcal{K}}\mathcal{S}\mathcal{K}\traj+\frac{1}{2}\risk\tran{\traj}\br{\tran{\mathcal{K}}\mathcal{R}\mathcal{K}+\mathcal{Q}}\traj}\diff{\ytraj}
\\
& = \frac{1}{c}\int \expb{-\frac{1}{2}\tran{\ytraj}\br{\mathcal{S}+\mathcal{S}\mathcal{K}\M+
\tran{\M}\tran{\mathcal{K}}\tran{\mathcal{S}}+
\tran{\M}\br{\tran{\mathcal{K}}\br{\risk\mathcal{R}-\mathcal{S}}\mathcal{K}+\risk\mathcal{Q}}\M}\ytraj}\diff{\ytraj} \\
& = \begin{cases}
&\infty \text{ if }  \mathcal{S}-\mathcal{S}\mathcal{K}\M-\tran{\M}\tran{\mathcal{K}}\tran{\mathcal{S}}\succeq
\tran{\M}\br{\tran{\mathcal{K}}\br{\risk\mathcal{R}-\mathcal{S}}\mathcal{K}+\risk\mathcal{Q}}\M \\
&\frac{\detb{\inv{\mathcal{S}-\mathcal{S}\mathcal{K}\M-\tran{\M}\tran{\mathcal{K}}\tran{\mathcal{S}}-
\tran{\M}\br{\tran{\mathcal{K}}\br{\risk\mathcal{R}-\mathcal{S}}\mathcal{K}+\risk\mathcal{Q}}\M}}}{\sqrt{\powb{2\pi}{\nc (\Nh-1)}\prod_{t=1}^{\Nh-1}\detb{\Unoise_t}} } \text{ otherwise}
\end{cases}
\end{align*}
When $\risk\mathcal{R}\succeq\mathcal{S}$, the above problem is a convex optimization problem and is equivalent to the following determinant maximization problem:
\begin{align*}
\maxi_{\Kb} \logb{\detb{\mathcal{S}-\mathcal{S}\mathcal{K}\M-\tran{\M}\tran{\mathcal{K}}\tran{\mathcal{S}}-
\tran{\M}\br{\tran{\mathcal{K}}\br{\risk\mathcal{R}-\mathcal{S}}\mathcal{K}+\risk\mathcal{Q}}\M}} \\
\text{Subject to } \mathcal{S}-\mathcal{S}\mathcal{K}\M-\tran{\M}\tran{\mathcal{K}}\tran{\mathcal{S}}-
\tran{\M}\br{\tran{\mathcal{K}}\br{\risk\mathcal{R}-\mathcal{S}}\mathcal{K}+\risk\mathcal{Q}}\M \succeq 0
\end{align*}


\subsection{Learning Neural Networks}

This approach can also be applied to learning neural networks. In this approach, the time-steps corresponds to layers of the neural network. In each step, the state (neural activations) are passed through a linear mapping and an component-wise nonlinear transfer function:
\[\s_{t+1}=h(K_t\s_t),\s_1=\alpha\]
where $h$ is applied component-wise (common examples include the sigmoid and tanh functions). To put this in our framework, we assume that the neural inputs are subject to noise, so that
\[\s_{t+1}=h(\yg_t),\yg_t=\ug_t+\noiseu_t,\ug_t=K_t\s_t.\]
Note that in our framework this corresponds to an $\Detff{\s_t}{\yg_t}{\noise_t}{t}=h(\yg_t)$, so the dynamics only depends on the (noisy) control input. The training data for the neural network are considered as external disturbances sampled from the true data distribution. The input is the initial state $\alpha$ and we would like to adjust the network weights $\Kb$ so that the final state $\s_{\Nh}$ matches the desired output, $\beta$.

The neural network training problem can be then phrased as a problem in our framework:
\[\mini_{\Kb} \ExP{(\alpha,\beta) \sim \mathbb{P}_{\text{data}},\noiseu_t \sim \Gauss{0}{\Unoise_t}}{\expb{\risk\costt\br{\s_{\Nh},\beta}+\sum_{i=1}^{\Nh-1} \risk\frac{\tran{\ug_t}\costu_t\ug_t}{2}}}\]

where $\costt$ is a loss function measuring the discrepancy between the desired output and that of the neural network. In practice the true distribution $\mathbb{P}_{\text{data}}$ is unknown and will be replaced by a sample average over training data. Our result says that as long as $\risk\costu_t \succeq \inve{\Unoise_t}$, the resulting problem is a convex optimization problem. Thus, we have a convex optimization problem for training neural networks with arbitrary architecture, transfer functions and data distributions! The way this differs from standard formulations of neural network training are:
\begin{itemize}
\item[a] The inputs to each layer must be made noisy by adding Gaussian noise $\Gauss{0}{\Sigma_t}$.
\item[b] The performance of the network is measured as the expectation over the added noise of an exponentiated augmented loss function: This has both a ``data'' term $\costt\br{\s_{\Nh},\beta}$ and a ``regularization'' term: $\sum_{t=1}^{\Nh-1} \frac{\tran{\s_t}\tran{K_t} \costu_t K_t\s_t}{2}$ which penalizes networks that have large activations or large weights.
\item[c] The noise added at each layer has to be ``sufficient'', that is, $\Sigma_t \succeq \frac{\inve{\costu_t}}{\risk}$
\end{itemize}

\subsection{Convex Reinforcement Learning}
As outlined in section \ref{sec:Algorithms}, stochastic gradient methods can be used to solve the convex optimization problems described in this paper. This is applicable even to the dynamical setting, leading to stochastic gradient methods for reinforcement learning and control. Stochastic approximation is an old idea in reinforcement learning and forms the basis of popular reinforcement learning algorithms like TD-learning, Q-learning and policy gradient algorithms \citep{szepesvari2010algorithms}. However, thus far, there were no guarantees made about the speed of convergence of these algorithms, particularly for continuous state problems.

Based on the results of section \ref{sec:Control}, we can derive policy optimization algorithms based on stochastic convex optimization that are guaranteed to converge to the optimal policy in polynomial time. The results can give rise to both model-free and model-based reinforcement learning algorithms, based on the type of gradient update used. We then develop 2 policy gradient learning algorithms for finite horizon problems (algorithms \ref{alg:StochGradPol},\ref{alg:DFStochGradPol}). Note that algorithm \ref{alg:StochGradPol} requires gradients of the dynamics (and hence a model of the dynamics) while algorithm \ref{alg:DFStochGradPol} is completely model-free and just uses roll-outs in order to compute policy gradients. 


%\subsection{Relationship to $\text{PI}^2$}

%Policy Improvements with Path Integrals \citep{theodorou2010generalized} is a recent policy optimization algorithm derived based on the theory of path integral control \citep{kappen05} and the related framework of linearly solvable MDPs \citep{Todorov09a}. It has been shown to be effective for several policy learning tasks in robotics and can work in a completely model-free way. Although derived for continuous-time problems, the implementation requires time-discretization and hence we can try to relate our approach to the $\text{PI}^2$ algorithm. TBD.

\begin{algorithm}[Stochastic Gradient Method]
 \begin{algorithmic}
 \State $\Kb \gets \Kb_0$
\For {$i = 1,\ldots,l$}
    \State $\hat{\costt}\gets 0$ \text{ (Cost Estimate for Rollout)}
    \For {$t = 1,\ldots,\Nh-1$} \text{ (Policy Rollout)}
        \State $\ug_t\gets K_t\feats\br{\s_t}$
        \State $\hat{\costt}\gets \hat{\costt}+\cost\br{\s_t}+\frac{\tran{\ug_t}\costu_t \ug_t}{2}$
        \State $\noiseu_t \sim \Gauss{0}{\Sigma_t}$    \text{ (Sample Control Noise)}
        \State $\noisew_t \sim \Pn$    \text{ (Sample System Noise)}
        \State $\s_{t+1} \gets \Detff{\s_t}{\ug_t+\noiseu_t}{\noisew_t}{t} $    \text{ (Simulate Dynamical System Step) }
    \EndFor
    \State $\hat{\costt}\gets \hat{\costt}+\costt_{\Nh}\br{\s_{\Nh}}$
 
    \State $\mathbf{G} \gets 0*\Kb$
    \State $\lambda \gets \nabla \cost_{\Nh}\br{\s_{\Nh}}$     
    \For {$t = \Nh-1,\ldots,1$} \text{ (Policy Gradient)}
        \State $G_t \gets \frac{\br{R_tK_t\s_t}\tranb{\feats\br{\s_t}}+\s_t\tranb{R_tK_t\feats\br{\s_t}}}{2}+\Diff{\s_{t+1}}{\ug_t}\lambda\tran{\feats\br{\s_t}}$
        \State $u_x \gets \tranb{K_t\Diff{\feats\br{\s_t}}{\s_t}}$
        \State $\lambda \gets \Diff{\costt\br{\s_t}}{\s_t}+u_xR_tK_t\feats\br{\s_t}+\br{\Diff{\s_{t+1}}{\s_t}+\tran{u_x}\Diff{\s_{t+1}}{\ug_t}}\lambda$
    \EndFor
    \State $\Kb \gets \Kb-\eta_i\br{\expb{\risk\hat{\costt}}}\mathbf{G}$
\EndFor
\end{algorithmic}
 \caption{Convex Stochastic Policy Gradient Method for \eqref{eq:OptC}}\label{alg:StochGradPol}
\end{algorithm}

\begin{algorithm}[Derivative-Free Stochastic Gradient Method]
 \begin{algorithmic}
  \State $\Kb \gets \Kb_0$
\For {$i = 1,\ldots,l$}
    \State $\hat{\costt}\gets 0$ \text{ (Cost Estimate for Rollout)}
    \For {$t = 1,\ldots,\Nh-1$} \text{ (Policy Rollout)}
        \State $\ug_t\gets K_t\feats\br{\s_t}$
        \State $\hat{\costt}\gets \hat{\costt}+\cost\br{\s_t}+\frac{\tran{\ug_t}\costu_t \ug_t}{2}$
        \State $\yg_t \sim \Gauss{\ug_t}{\Sigma_t}$    \text{ (Sample Noisy Control)}
        \State $\noisew_t \sim \Pn$    \text{ (Sample System Noise)}
        \State $\s_{t+1} \gets \Detff{\s_t}{\yg_t}{\noisew_t}{t} $    \text{ (Simulate Dynamical System Step) }
    \EndFor
    \State $\hat{\costt}\gets \hat{\costt}+\costt_{\Nh}\br{\s_{\Nh}}$

    \State $\mathbf{G} \gets 0*\Kb$
    \State $\lambda \gets \nabla \cost_{\Nh}\br{\s_{\Nh}}$
    \For {$t = \Nh-1,\ldots,1$} \text{ (Policy Gradient)}
        \State $G_t \gets \br{\inve{\Sigma_t}\br{\yg_t-\ug_t}+\risk \costu_t \ug_t}{\tranb{\feats\br{\s_t}}}$
        
    \EndFor
    \State $\Kb \gets \Kb-\eta_i\br{\expb{\risk\hat{\costt}}}\mathbf{G}$
\EndFor
\end{algorithmic}
 \caption{Derivative-Free Stochastic Gradient Method for \eqref{eq:OptC}}\label{alg:DFStochGradPol}
\end{algorithm}


%We can combine this approach with sampling based ideas used commonly in reinforcement learning to obtain model-free reinforcement learning methods with convexity guarantees - this is a first for reinforcement learning to the best of my knowledge.


